MoFa: A Unified Performance Modeling Framework for LLM Pretraining

The exponential growth in LLM scales, with parameters soaring from billions to trillions, has necessitated distributed pretraining across large clusters comprising thousands to tens of thousands of devices. While hybrid parallelization strategies enable such pretraining, the vast combinatorial strategy space introduces significant optimization challenges. Traditional manual tuning methods incur prohibitive trial-and-error costs, and existing performance modeling approaches exhibit critical limitations: they fail to comprehensively account for prevalent optimization features and ignore the substantial overhead imposed by essential fault tolerance mechanisms like checkpoint recovery in long-duration pretraining. To address these gaps, we propose MoFa, a novel pretraining performance modeling framework that unifies multi-dimensional optimization features and fault tolerance. MoFa incorporates an enhanced cost model to accurately capture the effects of key optimizations and integrates a fault tolerance model based on historical cluster reliability data. Besides, a MoFa-based tuning system is developed to explore optimal pretraining performance and potential bottlenecks in various scenarios. Extensive modeling evaluations demonstrate that MoFa can achieve high prediction accuracy across various scenarios. In addition, through comprehensive tuning experiments, our framework systematically reveals the key factors influencing pretraining performance under different configurations, which provides solid a priori guidance for LLM pretraining system design and deployment.

==> failure.tex <==
\section{Formulation}

\begin{align}
\label{ettr}Design
    ETTR = \frac{R}{R+U}
\end{align}

\begin{align}
\label{en}
    \mathbb{E}(N_f)=N_{nodes}r_f\left(R+\mathbb{E}\left(U\right)\right)
\end{align}

\begin{align}
\label{eu}
     \mathbb{E}(U)=\left(\mathbb{E}(N_f)+1\right)u_0+\mathbb{E}(N_f)\frac{\Delta t_{cp}}{2}+R\frac{w_{cp}}{\Delta t_{cp}}
\end{align}

from Eq.\ref{en}$\sim$ \ref{eu}, we have:
\begin{align}
\nonumber\mathbb{E}(N_f)=N_{nodes}r_f\left(R+\mathbb{E}\left(N_f\right)\left(u_0+\frac{\Delta t_{cp}}{2}\right)+u_0+R\frac{w_{cp}}{\Delta t_{cp}}\right)
\end{align}
Thus:
\begin{align}
\label{nfn}
\mathbb{E}(N_f)=\frac{N_{nodes}r_f\left(R+u_0+R\frac{w_{cp}}{\Delta t_{cp}}\right)}{1-N_{nodes}r_f\left(u_0+\frac{\Delta t_{cp}}{2}\right)}
\end{align}

Take Eq.\ref{nfn} into Eq.\ref{eu}:
\begin{align}
\label{finalu}
\nonumber\mathbb{E}(U)=&\frac{\mathbb{E}(N_f)}{N_{nodes}r_f}-R\\
=&\frac{\left(R+u_0+R\frac{w_{cp}}{\Delta t_{cp}}\right)}{1-N_{nodes}r_f\left(u_0+\frac{\Delta t_{cp}}{2}\right)}-R
\end{align}

Now, take Eq.\ref{finalu} into Eq.\ref{ettr}, we can get:
\begin{align}
    \mathbb{E}(ETTR)&\geq\frac{1}{1+\mathbb{E}(\frac{U}{R})}\nonumber\\
    &=\frac{1-N_{nodes}r_f\left(u_0+\frac{\Delta t_{cp}}{2}\right)}{1+\frac{u_0}{R}+\frac{w_{cp}}{\Delta t_{cp}}}
\end{align}

use $x$ denote $\Delta t_{cp}$, then:
\begin{align}
\label{ff}
    \mathbb{E}(ETTR)=f(x)\approx\frac{1-Nr(u+\frac{x}{2})}{1+\frac{w_{cp}}{x}}
    \\ \frac{\partial f}{\partial x}=\frac{-\frac{Nr}{2}\left(1+\frac{w}{x}\right)+\frac{w}{x^2}\left(1-Nru-\frac{Nrx}{2}\right)}{(1+\frac{w}{x})^2}
\end{align}
when Eq.\ref{ff}$=0$:
\begin{align}
    \Delta t_{cp}=x=-w+\sqrt{w^2-2wu+\frac{2w}{Nr}}
\end{align}

 \begin{figure}[h!]%htbp
 \centering
 \subfigure[N]{
 \includegraphics[width=0.48\linewidth]{./figures/N.pdf}}
  \subfigure[r]{
  \includegraphics[width=0.48\linewidth]{./figures/r.pdf}}


  \subfigure[u]{
  \includegraphics[width=0.48\linewidth]{./figures/u.pdf}}
  \subfigure[w]{
  \includegraphics[width=0.48\linewidth]{./figures/w.pdf}}
 \caption{
The trend of the optimal saving interval (minutes) with configuration changes.
 }
 \label{com}
 \end{figure}

 从以上推导可以看到两个现象：1）ETTR的下界与训练过程中保存ckpt耗时、保存ckpt间隔、总节点数、故障率、初始化时间相关。后续我们会从数值角度来揭示这些变量对ETTR的精确影响。2）值得注意的是，训练任务的计算总耗时并不影响ETTR，这反映ETTR是对基础设施能力的一个良好描述。

 下面我们对ETTR的公式进行求导，可以找到当ETTR达到最大值时的最优保存时间间隔为：
 \begin{align}
    \Delta t_{cp}=x=-w+\sqrt{w^2-2wu+\frac{2w}{Nr}}
\end{align}

从中可以看到：1）当故障率出现$(\frac{1}{Nr}-u)^2\leq 1$时，不存在最优值，这暗示了，当故障发生率非常高时（\textcolor{red}{例如32节点场景下，约45次故障每节点日）}，存储ckpt已经失去意义，此时不保存ckpt才能使ETTR最大化。2）不同的训练过程变量对最终ETTR的重要性不一，其中初始化时间u对ETTR的影响最小。

如图~\ref{com}所示，我们展示了不同因素对最优保存间隔的影响，可以看到,N、r、w对最优间隔有显著影响，而u对最优间隔的影响较小，当u从0秒变化到300s时，最优保存间隔只变化了0.01分钟。我们也画出了各种参数下的最优ETTR，如图~\ref{ettrfig},可以看到压缩初始化时间u对整体的ETTR收益最小。

\begin{figure}[h!]%htbp
    \centering
    \subfigure[N]{
    \includegraphics[width=0.48\linewidth]{./figures/ettr-N.pdf}}
     \subfigure[r]{
     \includegraphics[width=0.48\linewidth]{./figures/ettr-r.pdf}}
   
   
     \subfigure[u]{
     \includegraphics[width=0.48\linewidth]{./figures/ettr-u.pdf}}
     \subfigure[w]{
     \includegraphics[width=0.48\linewidth]{./figures/ettr-w.pdf}}
    \caption{
   各参数对应的最优ETTR
    }
    \label{ettrfig}
    \end{figure}


==> notationtable.tex <==
\begin{table}[notationtable]
\begin{tabular}{ccc}
                        & 符号 & 含义   \\ \hline
\multirow{2}{*}{模型结构参数} & L  & 模型层数 \\
                        & A  & B    \\ \hline
\multirow{3}{*}{并行配置参数} & t  & TP大小 \\
                        & p  & PP大小 \\
                        & C  & D    \\ \hline
\multirow{2}{*}{硬件参数}   & E  & F    \\
                        & G  & H    \\ \hline
\multirow{2}{*}{耗时划分}   & Z  & Y    \\
                        & K  & M    \\ \hline
\end{tabular}
\end{table}

==> temp.tex <==
% \begin{align}
%     T_{\mathrm{overlap}}^{\mathrm{EP}} = \max \left(\alpha _\mathrm{overlap}^{\mathrm{EP}}T^{\mathrm{EP}}, \beta _\mathrm{overlap}^{\mathrm{EP}}T_{\mathrm{noEP}}^{\mathrm{BWD}} \right)+\max \left(\alpha _\mathrm{overlap}^{\mathrm{EP}}T^{\mathrm{EP}}, \beta _\mathrm{overlap}^{\mathrm{EP}}T_{\mathrm{noEP}}^{\mathrm{FWD}} \right)
% \end{align}

% \begin{align}
% \nonumber
%     T_{\mathrm{overlap}}^{\mathrm{CP}} = & \frac{1}{c}T_1^{\mathrm{CP}}+\max\left(\alpha _\mathrm{overlap}^{\mathrm{CP}}\sum\nolimits_{i=2}^{v}T_i^{\mathrm{CP}}, \beta _\mathrm{overlap}^{\mathrm{CP}}T^{\mathrm{attention}_\mathrm{fwd}} \right)+ \\
%     &\max \left(\alpha _\mathrm{overlap}^{\mathrm{CP}}T^{\mathrm{CP}}, \beta _\mathrm{overlap}^{\mathrm{CP}}T^{\mathrm{attention}_\mathrm{bwd}} \right)
% \end{align}


%TP通信：
% \begin{align}
% T_{\mathrm{overlap}}^{\mathrm{TP}_\mathrm{ag}} = \frac{1}{s_n} \min \Biggl(T^{\mathrm{TP}_\mathrm{ag}},T^{\mathrm{Linear}_\mathrm{QKV}} \Biggr)+ 
% \max \Biggl( \alpha ^\mathrm{TP_\mathrm{ag}}_\mathrm{overlap}T^{\mathrm{TP}_\mathrm{ag}}, \beta ^\mathrm{TP_\mathrm{ag}}_\mathrm{overlap}T^{\mathrm{Linear}_\mathrm{QKV}} \Biggr)
% \end{align}
% \begin{align}
% T_{\mathrm{overlap}}^{\mathrm{TP}_\mathrm{rs}} = \frac{1}{s_n} \min \Biggl(T^{\mathrm{TP}_\mathrm{rs}},T^{\mathrm{Linear}_\mathrm{O}} \Biggr)+ 
% \max \Biggl( \alpha ^\mathrm{TP_\mathrm{rs}}_\mathrm{overlap}T^{\mathrm{TP}_\mathrm{rs}}, \beta ^\mathrm{TP_\mathrm{rs}}_\mathrm{overlap}T^{\mathrm{Linear}_\mathrm{O}} \Biggr)
% \end{align}

\subsubsection{计算-通信并行代价模型}
计算-通信并行是大模型分布式训练中常用的优化技术，该技术的优化原理是将并行组通信和其无数据依赖的计算并行执行以减少通信开销，如图1所示，对于该类优化，统一的costmodel可以公式化为如下形式：
\begin{align}
    T=max\left(\alpha\times T^{commu},\beta\times T^{comp}\right)
\end{align}
其中$\alpha$和$\beta$分别为计算和通信掩盖后的通信耗时增长系数和计算耗时增长系数，这通常由硬件资源冲突导致，并能够通过大量实验预估，$T^{comp}$为参与掩盖的计算耗时，$T^{commu}$为参与掩盖的通信耗时。参与掩盖的计算必须和通信无数据依赖，否则无法进行Overlap。

一般来说，不同的并行组通信均可以设计实现计算-通信掩盖，不同的Overlap影响基础性能维度不同。在公式(1)引导下，我们对主流的并行组通信掩盖策略进行代价模型建模。

TP Overlap：如图2所示，TP通信存在每层，一般通过相邻的矩阵乘和TP通信切成多份交叠掩盖，减少TP通信耗时，例如QKV Linear和TP ag Overlap，O Linear和TP rs Overlap。基于该设计，一层前向和一层反向中TP通信和计算Overlap暴露的有效耗时建模分别为如下：
\begin{align}
T_{\mathrm{overlap}}^{\mathrm{TP}_\mathrm{ag}} = \frac{1}{s_n} \min \Biggl(T^{\mathrm{TP}_\mathrm{ag}},T^{\mathrm{Linear}_\mathrm{QKV}} \Biggr)+ 
\max \Biggl( \alpha ^\mathrm{TP_\mathrm{ag}}_\mathrm{overlap}T^{\mathrm{TP}_\mathrm{ag}}, \beta ^\mathrm{TP_\mathrm{ag}}_\mathrm{overlap}T^{\mathrm{Linear}_\mathrm{QKV}} \Biggr)
\end{align}

\begin{align}
T_{\mathrm{overlap}}^{\mathrm{TP}_\mathrm{rs}} = \frac{1}{s_n} \min \Biggl(T^{\mathrm{TP}_\mathrm{rs}},T^{\mathrm{Linear}_\mathrm{O}} \Biggr)+ 
\max \Biggl( \alpha ^\mathrm{TP_\mathrm{rs}}_\mathrm{overlap}T^{\mathrm{TP}_\mathrm{rs}}, \beta ^\mathrm{TP_\mathrm{rs}}_\mathrm{overlap}T^{\mathrm{Linear}_\mathrm{O}} \Biggr)
\end{align}
其中$s_n$为矩阵乘和TP通信切分数。

PP Overlap：如图3所示，PP通信在一个微批次处理完后执行，一般利用下一个微批次的前向过程或者反向过程掩盖相邻的PP通信过程，一般作用在steady阶段。在PP Overlap的优化下，交叠式1F1B steady阶段中PP通信和计算Overlap暴露的有效耗时建模为如下：

DP Overlap：如图4所示，DP通信在所有微批次前向反向全部执行完后进行梯度的DP组通信。一般来说，在大规模分布式训练中，会采用分布式优化器（zero1）来减少显存，此时DP通信包含梯度reduce-scatter(rs)和参数allgather(ag)。在交叠式1F1B中一般利用chunk i的反向过程掩盖chunk i+1的梯度rs，利用chunk i的前向过程掩盖chunk i+1的参数ag。基于该设计，带有DP Overlap特性的DP通信和计算暴露的有效耗时建模为如下：
\begin{align}
    T_{\mathrm{overlap}}^{\mathrm{DP}} =  T_{\mathrm{chunk}_1}^{\mathrm{DP}_{\mathrm{rs}}} + T_{\mathrm{chunk}_1}^{\mathrm{DP}_{\mathrm{ag}}} + &\max \Biggl(\alpha _\mathrm{overlap}^{\mathrm{DP}_{\mathrm{rs}}}\sum\nolimits_{j=2}^{v}T_{\mathrm{chunk}_j}^{\mathrm{DP}_{\mathrm{rs}}}, \beta _\mathrm{overlap}^{\mathrm{DP}_{\mathrm{rs}}}\frac{v-1}{v}LT^{\mathrm{BWD}}\Biggr) + 
    \\ \nonumber
    & \max \Biggl(\alpha _\mathrm{overlap}^{\mathrm{DP}_{\mathrm{rs}}}\sum\nolimits_{j=2}^{v}T_{\mathrm{chunk}_j}^{\mathrm{DP}_{\mathrm{rs}}}, \beta _\mathrm{overlap}^{\mathrm{DP}_{\mathrm{rs}}}\frac{v-1}{v}LT^{\mathrm{FWD}}\Biggr)   
\end{align}

EP Overlap：如图5所示，EP通信掩盖通常采用类似DualPipe中前向和反向相互掩盖的策略，在一次前向传播过程一次反向传播过程的调度中应用。具体来说，在一层中，将前向的计算和反向的EP通信进行掩盖，将反向的计算和前向的EP通信进行掩盖。基于该设计下，EP通信和计算Overlap后有效暴露耗时建模为如下：
\begin{align}
    T_{\mathrm{overlap}}^{\mathrm{EP}} = \max \left(\alpha _\mathrm{overlap}^{\mathrm{EP}}T^{\mathrm{EP}}, \beta _\mathrm{overlap}^{\mathrm{EP}}T_{\mathrm{noEP}}^{\mathrm{BWD}} \right)+\max \left(\alpha _\mathrm{overlap}^{\mathrm{EP}}T^{\mathrm{EP}}, \beta _\mathrm{overlap}^{\mathrm{EP}}T_{\mathrm{noEP}}^{\mathrm{FWD}} \right)
\end{align}
其中，符号说明

CP Overlap：如图6所示，CP通信通常采用ring方式进行token的获取与通信掩盖，用第i次attention计算掩盖第i+1批序列的p2p通信。在该设计下，带有CP Overlap特性的CP通信耗时建模为：
\begin{align}
\nonumber
    T_{\mathrm{overlap}}^{\mathrm{CP}} = & \frac{1}{c}T_1^{\mathrm{CP}}+\max\left(\alpha _\mathrm{overlap}^{\mathrm{CP}}\sum\nolimits_{i=2}^{v}T_i^{\mathrm{CP}}, \beta _\mathrm{overlap}^{\mathrm{CP}}T^{\mathrm{attention}_\mathrm{fwd}} \right)+ \\
    &\max \left(\alpha _\mathrm{overlap}^{\mathrm{CP}}T^{\mathrm{CP}}, \beta _\mathrm{overlap}^{\mathrm{CP}}T^{\mathrm{attention}_\mathrm{bwd}} \right)
\end{align}
其中，符号说明


\textbf{\subsubsection{通信亲和代价模型}
在通信建模中，通信带宽对通信性能至关重要，在实际部署中，由于不同并行组通信的通行量和通信次数差异较大，不同的并行组部署会导致通信带宽差异，进而影响端到端性能，根据实际场景选择性能最优的通信策略称之为通信亲和策略。 目前业界通信亲和策略根据通信量默认按照TP-CP-EP-DP/PP-PP/DP的亲和政策。根据DP和PP次序，将亲和政策分为两类：DP亲和和PP亲和。在DP亲和下，DP通信带宽会优先放到高带宽域。反之，在PP亲和策略下 ，PP通信带宽会优先放到高带宽域。因此通信亲和代价模型可以统一建模为亲和并行组通信带宽的建模。

DP亲和：
\begin{align}
B^\mathrm{DP}=\left\{\begin{matrix}B^\mathrm{intranode} & if\ tced\leqslant N\\ B^\mathrm{internode}  & else\end{matrix}\right. & 
\end{align}
PP亲和：
\begin{align}
B^\mathrm{PP}=\left\{\begin{matrix}B^\mathrm{intranode} & if\ tcep\leqslant N\\ B^\mathrm{internode}  & else\end{matrix}\right. & 
\end{align}
}


\textbf{服务器因素}：
\begin{enumerate}
\item Device-to-Host(D2H)带宽$B^\mathrm{H2D}$：device向host传递数据的能力，影响训练中激活值卸载等操作；
\item Host-to-Device(H2D)带宽$B^\mathrm{D2H}$：host向device传递数据的能力，影响训练中激活值预取等操作；
\item 磁盘加载带宽$Bdisk^\mathrm{Load}$：决定从磁盘加载训练数据、模型检查点等的速度；；
\item 磁盘写入带宽$Bdisk^\mathrm{Write}$：影响检查点保存、日志写入等持久化操作的性能；
\item CPU内存$M^\mathrm{CPU}$：限制了可在主机端缓存的数据量，进一步影响 Device 与 Host 间数据交换的调度策略；
\item CPU主频$F^\mathrm{CPU}$：表征CPU在理想状态下每秒可执行的浮点运算次数（FLOPS），是CPU上计算的基础指标
\end{enumerate}

\textbf{GPU芯片因素}：
\begin{enumerate}
\item规格算力$P^\mathrm{GPU}$：表征GPU在理想状态下每秒可执行的浮点运算次数（FLOPS），是GPU计算的基础指标；
\item GPU内存$M^\mathrm{GPU}$：决定了单卡可驻留的模型规模与批量数据大小，直接影响是否需采用模型并行等策略；
\end{enumerate}

\textbf{组网因素}：
\begin{enumerate}
\item 节点形态$N$：指单个物理节点中所包含的GPU数量，影响局部通信与全局通信的拓扑结构；
\item 节点内物理带宽$Bbus^\mathrm{intranode}$：节点内的传输能力，影响训练中节点间通信时延指同一节点内多GPU之间的通信带宽，影响All-Reduce、All-Gather等集合通信操作的延迟；
\item 节点间物理带宽$Bbus^\mathrm{internode}$：跨节点之间的网络传输能力，通常取决于InfiniBand(IB)或高速以太网配置，制约数据并行训练中的梯度同步效率；
\end{enumerate} 
通过以上硬件因素的抽象与统一表示，为后续构建统一多维优化特性和动态故障容错的性能模型提供了理论基础。此外，和训练算法相关的参数按照如下进行符号化：
{\color{red}补充个符号表}。


\subsection{Basic Performance Cost Model}

在本章节中，我们介绍训练系统基础代价模型$\mathrm{CostModel}_\mathrm{base}$，它数学上表征了训练系统最基本的组件和流程。图\ref{one-step}展示了当前大模型训练系统时序示意图，根据该流程我们将$\mathrm{CostModel}_\mathrm{base}$归纳为五方面：模型结构拆解，算子和通信耗时建模、层级耗时建模、流水线级耗时建模、优化器耗时建模和显存占用建模。

\textbf{模型结构拆解}：目前的LLM绝大部分采用decoder-only架构，该架构中当前应用最为广泛的是Dense结构，例如LLaMA1/2/3系列模型，和MoE结构，例如DeepSeek。我们将模型架构分成三级，其中Dense，Moe的第一级第二级架构相同，第三级Dense和Moe在MLP处有差异。表格x展示了大部分Dense和Moe结构，其中attention部分以MHA为例进行展示。实际中，attention模块可选MHA，GQA，MQA和MLA等结构，这会影响FLOPs和激活值大小。

\textbf{算子和通信耗时建模}：算子和通信数据作为大模型分布式训练的基石，对训练性能有着严重的影响。对算子和通信耗时建模主要有两种方法：理想假设和Profiling获取。在本文中，考虑基于profiling的方式数据精度更高，我们采用基于profiling方式实现对算子算力$P^{comp}$和通信算法带宽$B^{commu}$建模，不同模块的算子和通信建模为如下：
\begin{align}
\label{comp}
    T_i^{comp}=S_i^{comp}/P_i^{comp}
\end{align}
\begin{align}
\label{commu1}
    T_j^{commu}=S_j^{commu}/B_j^{commu}
\end{align}
其中$S_i^{comp}$为第$i$个计算模块的计算量，$P_i^{comp}$为profiling获取到的算子数据，$S_j^{commu}$为第$j$个通信模块的通信量，$B_j^{commu}$为profiling获取到的通信带宽数据。一般来说，采用少量硬件资源测试不同shape的计算模块便可以获取计算算力，相反，通信需要同等评估规模数据来采集通信带宽数据，这对于超大规模集群评估是无法满足要求的。为了解决该问题，我们首先在少量硬件资源上测试通信带宽数据，然后根据专家经验对带宽进行调整。按照这种方式，\ref{commu1}转化为如下：
\begin{align}
\label{commu2}
    T_j^{commu}=\frac{S_j^{commu}}{\beta_j B_j^{commu}}
\end{align}

\input{Table/3/modelarchitecture}

\textbf{显存代价模型}：大模型训练中显存分为两类：静态显存和动态显存。静态显存主要包含三部分：权重参数、权重梯度、优化器状态，每部分显存占用和设备上参数量以及数据精度相关，静态显存建模如下：
\begin{align}
\label{staticmem}
M^\mathrm{sta}=\underbrace{D_t^\mathrm{para}vl\sum_i^{m_n}S_i^\mathrm{para}}_{\mathrm{Parameter}}
+\underbrace{D_t^\mathrm{grad}vl\sum_i^{m_n}S_i^\mathrm{para}}_{\mathrm{Grad}}+\underbrace{4D_t^\mathrm{opt}vl\sum_i^{m_n}S_i^\mathrm{para}}_\mathrm{{Optimizer}}
\end{align}
其中$S_i^\mathrm{para}$为每个设备上第i个模块需要保存在GPU上的参数量，$D_t^\mathrm{para}$，$D_t^\mathrm{grad}$和$D_t^\mathrm{opt}$分别为参数，梯度和优化器状态的数据类型。

动态显存是指在训练过程中增加的显存，一般来自于训练中间激活值，其是指模型前向传播中保存用于反向传播的中间值。此外，如图x所示，流水线调度一般采用“warmup-steady-cooldown”方式进行微批次调度，由于warmup阶段只存在前向过程，会不断累积激活值直到warmup阶段结束。基于该设计下，整个训练系统的中间激活值显存峰值建模为如下：
\begin{align}
\label{actmem}
M^\mathrm{act}=\left(vp+p-2r_{pp}-1 \right)\sum_i^{m_n}M_i^\mathrm{act}
\end{align}
其中，$M_i^\mathrm{act}$表示计算模块$i$的激活值大小，$r_{pp}$表示当前PP编号。根据\ref{actmem}，可以得出一般第一个PP stage上显存压力最大，为$\left(vp+p-1 \right)\sum_i^{m_n}M_i^\mathrm{act}$。

基于\ref{staticmem}和\ref{actmem}，我们可得到训练系统中显存占用峰值为：
\begin{align}
\label{allmem}
M_\mathrm{peak}=M^\mathrm{sta}+M^\mathrm{act}
\end{align}

\textbf{层级代价模型}：层级代价模型是指对一层transformer层前向过程和反向过程进行耗时建模。根据模型结构表x，我们对模型一层transformer层进行统一的层级建模：
\begin{align}
\label{baseFWD}
T^\mathrm{FWD}=\sum\nolimits_{i=1}^{m_n} T_i^\mathrm{comp}+\sum\nolimits_{j=1}^{c_n} T_j^\mathrm{commu}
\end{align}
\begin{align}
\label{baseBWD}
    T^\mathrm{BWD}=\sum\nolimits_{i=1}^{m_n} T_i^\mathrm{comp_{BWD}}+\sum\nolimits_{j=1}^{c_n} T_j^\mathrm{commu}
\end{align}
其中$T_i^\mathrm{comp}$为计算模块$i$的前向传播耗时，$T_i^\mathrm{comp_{BWD}}$为计算模块$i$的反向传播耗时，$T_j^\mathrm{commu}$为通信模块$j$的耗时。

\textbf{流水线级代价模型}: 流水线代价模型是在微批次视角对PP流水调度进行建模。同主流建模技术~\cite{yuan2024accelerating}，本文考虑主流的交叠式1F1B流水线调度，其代价模型为：
\begin{align}
\label{ppwarmup}
T^\mathrm{Warmup} =p(T^\mathrm{Embed}+lT^\mathrm{FWD}+T^\mathrm{PP})+(vp-p-1)(lT^\mathrm{FWD}+T^\mathrm{PP})
\end{align}
\begin{align}
\label{ppsteady}
\nonumber
T^\mathrm{Steady}=&p(lT^\mathrm{FWD}+T^\mathrm{Head}++T^\mathrm{Head_{BWD}}+lT^\mathrm{BWD})
\\ &+(m_b-p)(vlT^\mathrm{FWD}+T^\mathrm{Head}+T^\mathrm{Head_{BWD}}+lT^\mathrm{BWD}) \\&+ (4m_bv-2m_b+2p-2)T^\mathrm{PP}
\end{align}
\begin{align}
\label{ppcooldown}
T^\mathrm{Cooldown}=p(T^\mathrm{Embed_{BWD}}+lT^\mathrm{BWD}+T^\mathrm{PP})+ (vp-p-1)(lT^\mathrm{BWD}+T^\mathrm{PP})
\end{align}
\begin{align}
    \label{pipeline}
    T^\mathrm{Pipeline} = T^\mathrm{Warmup} + T^\mathrm{Steady} + T^\mathrm{Cooldown}
\end{align}
其中$T_\mathrm{Embed}$和$T^\mathrm{Embed_{BWD}}$分别表示为Embedding模块前向传播和反向传播耗时，$T_\mathrm{Head}$和$T^\mathrm{Head_{BWD}}$分别表示为Head模块前向传播和反向传播耗时。

\textbf{优化器级建模}：优化器调度主要包含两个过程：DP通信和参数更新，建模为如下：
\begin{align}
\nonumber
\label{optimizer}
    T^\mathrm{Opt}&=T^\mathrm{DP}+T^\mathrm{WU} \\
    & = \frac{D_t^\mathrm{grad}vl\sum_i^{m_n}S_i^\mathrm{para}}{B^\mathrm{DP}}+\frac{vl\sum_i^{m_n}S_i^\mathrm{para}}{P^\mathrm{Opt}}
\end{align}
其中$P^\mathrm{Opt}$表示优化器参数更新的算力。

基于\ref{baseFWD}$\sim$\ref{optimizer}，一个step下训练端到端耗时建模为：
\begin{align}
\label{e2ebase}
    T^\mathrm{E2E}=T^\mathrm{Pipeline}+T^\mathrm{Opt}
\end{align}

\subsection{Multi-Dimensional Optimizations advanced Performance Cost Model}
在实际的大模型训练中，并行策略和优化特性同时影响训练效率。不同的优化特性作用于基础建模不同的层级上，影响并行策略的最优选择。为了统一优化特性对性能的影响，我们在基础代价模型基础上引入多维优化特性建模增强，以更精确和更全面地建模训练系统性能。$CostModel_\mathrm{Mo}$是一个统一的建模框架，在\ref{e2ebase}基础上引入当前主流的各类优化特性，涵盖层级优化(Layer-Level Optimization, LO)、流水线级优化(Pipeline-Level Optimization, PO)、优化器级优化(Optimizer-Level Optimization, OO)和显存级优化(Memory-Level Optimizer, MO)，表示为如下：
\begin{align}
\label{costmodelmofa}
    CostModel_\mathrm{Mo} = CostModel_\mathrm{base}\left(LO,PO,OO,MO\right)
\end{align}
针对每类优化特性，我们设计了代价模型用于描述对训练系统性能的影响。

\subsubsection{层级优化建模}
层级优化是指影响\ref{baseFWD}和\ref{baseBWD}的优化，包括层级通信带宽提升、层级计算算力提升和层级计算-通信掩盖设计。层级通信带宽提升是优化通信算法提升通信带宽，层级计算算力优化是指优化计算实现算法以提高计算算力，在建模中，为了统一表达这两部分对性能的影响，我们通过引入比例系数建模这两种优化的效果，如下：
\begin{align}
\label{suanzi-up}
P_i^{\mathrm{comp}}=\lambda_i^\mathrm{comp}P_i^\mathrm{comp} 
\end{align}
\begin{align}
\label{tongxin-up}
B_j^{\mathrm{commu}}=\lambda_j^\mathrm{commu}B_j^\mathrm{commu}
\end{align}
将\ref{suanzi-up}和\ref{tongxin-up}分别代入\ref{comp}和\ref{commu2}以表征算力提升和带宽提升对性能影响。

层级通信与计算掩盖设计根据层级通信类型包含三类：TP通信-计算掩盖，CP通信-计算掩盖和EP通信-计算掩盖，每类掩盖原理不同，我们根据设计原理对每种掩盖策略进行建模。

TP Overlap一般通过相邻的矩阵乘算子和TP通信切成多个阶段进行交叠掩盖，例如将QKV生成矩阵乘操作和TP ag通信进行交叠掩盖。在将该设计下，TP通信和计算掩盖暴露的有效耗时建模表示为如下：
\begin{align}
\label{tp-overlap-costmodel}
T_i^{\mathrm{comp}} + T_j^{\mathrm{TP}} = \frac{1}{s_n} \min \Biggl(T_i^{\mathrm{comp}},T_j^{\mathrm{TP}} \Biggr)+ 
\max \Biggl( \alpha_i ^\mathrm{comp}T_i^{\mathrm{comp}}, \beta_j ^\mathrm{TP}T_j^\mathrm{TP} \Biggr)
\end{align}
其中$s_n$为切分的阶段数，$T_j^{\mathrm{TP}}$和$T_i^{\mathrm{comp}}$分别为第$j$个TP通信和参与掩盖TP通信的第$i$个计算模块，$\alpha_i ^\mathrm{comp}$和$\beta_j ^\mathrm{TP}$分别掩盖时第$i$个计算和第$j$个TP通信的耗时增长系数，通常是由于硬件资源抢占导致。

CP Overlap通常采用ring-attention的方式进行设计，其原理为用第i次attention计算掩盖第i+1批序列的peer2peer通信。在将该设计下，CP通信-计算Overlap暴露的有效耗时建模为如下：
\begin{align}
\label{cp-overlap-costmodel}
T_i^{\mathrm{attention}} + T_j^{\mathrm{CP}} = \frac{1}{c} \min \Biggl(T_i^{\mathrm{attention}},T_j^{\mathrm{CP}} \Biggr)+ 
\max \Biggl( \alpha_i ^\mathrm{attention}T_i^{\mathrm{attention}}, \beta_j ^\mathrm{CP}T_j^\mathrm{CP} \Biggr)
\end{align}
其中$T_i^{\mathrm{attention}}$和$T_j^{\mathrm{CP}}$分别表示ring-attention中第$i$次attention计算和第$j$次CP通信，$\alpha_i ^\mathrm{attention}$和$\beta_j ^\mathrm{CP}$分别掩盖时第$i$计算和第$j$的CP通信的耗时增长系数。

EP Overlap：EP通信掩盖通常采用类似前向和反向相互掩盖的设计。具体来说，在一层中，将前向传播的计算和反向传播的EP通信进行相互掩盖，将反向传播的计算和前向传播的EP通信进行相互掩盖。在该设计下，EP通信和计算Overlap后有效暴露耗时统一建模为如下：
\begin{align}
\label{ep-overlap-costmodel}
    \sum\nolimits_{i=1}^{m_n}T_i^{\mathrm{comp}} + \sum\nolimits_{j=1}T_j^{\mathrm{EP}} = \max \left(\alpha _i^{\mathrm{comp}}\sum\nolimits_{i=1}^{m_n}T_i^{\mathrm{comp}}, \beta _j^{\mathrm{EP}}\sum\nolimits_{j=1}^{c_n}T_j^{\mathrm{EP}}\right)
\end{align} 
其中$T_j^{\mathrm{EP}}$和$T_i^{\mathrm{comp}}$分别为第$j$个EP通信和参与掩盖EP通信的第$i$个计算模块，$\alpha_i ^\mathrm{comp}$和$\beta_j ^\mathrm{EP}$分别掩盖时第$i$计算和第$j$的EP通信的耗时增长系数。

将\ref{suanzi-up}$\sim$\ref{ep-overlap-costmodel}应用在\ref{baseFWD}和\ref{baseBWD}上可得到层级优化增强的代价模型，以表征层级优化对一层耗时影响。

\subsubsection{流水线级优化建模}
流水线级优化指影响\ref{pipeline}的优化。流水线级优化包含层级优化和$T^\mathbf{PP}$相关优化。层级优化在上一小节已介绍，将层级优化带入到\ref{pipeline}中可以得到层级优化对流水线的性能影响。本小节着重说明$T^\mathbf{PP}$相关优化建模，主要分为PP通信带宽提升和PP-计算掩盖设计。PP通信带宽提升建模和\ref{commu2}保持一致。

PP-计算掩盖设计利用下一个微批次的前向过程或者反向过程掩盖相邻的PP通信过程，主要作用在steady 阶段，我们将该PP-计算掩盖建模为如下：
\begin{align}
\label{PPOverlap}
    T^{\mathrm{PP}} = \max \Biggl(0, \beta_j^{\mathrm{PP}}T^{\mathrm{PP}}-\alpha_k\sum\nolimits_{k=1}^{l}T_k^\mathrm{onelayer} \Biggr)
\end{align}
其中$T_k^\mathrm{onelayer}$表示第$k$层耗时，前向传播过程掩盖PP通信时代入\ref{baseFWD}，反向传播过程掩盖PP通信时代入\ref{baseBWD}，$\beta_j^{\mathrm{PP}}$和$\alpha_k$分别为第$j$个PP模块和第$k$层计算的耗时增长系数。将\ref{PPOverlap}带入\ref{ppsteady}中来表征反应PP-计算掩盖对流水线性能的影响。

\subsubsection{优化器优化建模}
优化器优化指影响\ref{optimizer}的优化，主要分为两部分：DP通信优化和参数更新加速。
DP通信优化分为两种：DP通信带宽提升和DP通信计算掩盖设计。DP通信带宽提升的建模和\ref{commu2}保持一致。DP通信-计算掩盖设计一般采用流水线计算过程掩盖DP通信。具体来说，用流水线Cooldown阶段掩盖梯度的rs，即第$i$个虚拟管道的反向过程掩盖第$i+1$个虚拟管道梯度的rs，用Warmup阶段掩盖参数的ag，即第$i$个虚拟管道的前向过程掩盖第$i+1$个虚拟管道参数的ag，我们将该设计建模为如下：
\begin{align}
\label{dpoverlap}
    T^{\mathrm{DP}} =  T_{\mathrm{chunk}_1}^{\mathrm{DP}_{\mathrm{rs}}} + T_{\mathrm{chunk}_1}^{\mathrm{DP}_{\mathrm{ag}}} + &\max \Biggl(\alpha ^{\mathrm{DP}_{\mathrm{rs}}}\sum\nolimits_{i=2}^{v}T_{\mathrm{chunk}_i}^{\mathrm{DP}_{\mathrm{rs}}}, \beta ^{\mathrm{BWD}}pl(v-1)T^{\mathrm{BWD}}\Biggr) + 
    \\ \nonumber
    & \max \Biggl(\alpha ^{\mathrm{DP}_{\mathrm{ag}}}\sum\nolimits_{j=2}^{v}T_{\mathrm{chunk}_j}^{\mathrm{DP}_{\mathrm{ag}}}, \beta ^{\mathrm{FWD}}pl(v-1)T^{\mathrm{FWD}}\Biggr)
\end{align}
其中$T_{\mathrm{chunk}_i}^{\mathrm{DP}_{\mathrm{rs}}}$和$T_{\mathrm{chunk}_j}^{\mathrm{DP}_{\mathrm{ag}}}$分别为第$i$个虚拟管道rs和第$j$个虚拟管道ag耗时，
$\alpha ^{\mathrm{DP}_{\mathrm{rs}}}$和$\beta ^\mathrm{BWD}$分别为DP rs和反向传播的耗时增加系数，$\alpha ^{\mathrm{DP}_{\mathrm{ag}}}$和$\beta ^\mathrm{FWD}$分别为DP ag和前向传播的耗时增加系数。

参数更新加速属于算子优化，主要是优化参数更新算法提升算力，建模和\ref{suanzi-up}保持一致。
% \begin{align}
% \label{update-optimization}
% P^\mathrm{Opt} = \alpha P^\mathrm{Opt}
% \end{align}

将\ref{dpoverlap}和\ref{suanzi-up}带入\ref{optimizer}用于描述优化器调度优化对优化器耗时的影响。

\subsubsection{显存优化建模}
随着模型训练规模的不断扩大，对显存的需求也日益增长，显存优化已成为一项关键的训练加速手段。当前主流分布式训练框架普遍支持多种显存节省技术，可归纳为两类：优化器状态显存优化和激活值显存优化。然而，显存优化在节省显存的同时，往往会对训练速度产生影响。为量化此类优化的实际效果，我们针对上述两类策略，分别建立了显存占用与训练性能的代价模型。

\textbf{优化器静态显存优化}：优化策略包含分布式优化器和CPU优化器，二者都可以节省大量优化器状态显存占用，但对性能影响不同。分布式优化器通过将优化器状态平分到DP组，减少每个DP上优化器显存占用，每个DP负责维护1/DP的参数更新，因此也可以减少(DP-1)/DP的参数更新耗时。基于此，分布式优化器特性下显存和性能建模如下：
\begin{align}
\label{distributed-optimizer}
    & M^{\mathrm{optimizer}} = 4D_t^\mathrm{opt}vl\sum_i^{m_n}S_i^\mathrm{para}/{d} \\
    & T_\mathrm{update} = T_\mathrm{update}/{d}
\end{align}
其中$T_\mathrm{update}$为优化器参数更新耗时。

CPU优化器将优化器梯度卸载至CPU，在CPU上执行参数更新过程，更新完后再将参数放回GPU上，可以减少接近100\%的优化器显存，但会引入大量H2D和D2H耗时和CPU参数更新耗时，我们将CPU优化器特性下显存和性能建模如下：
\begin{align}
\label{cpuadam}  
    & M^{\mathrm{optimizer}} = \max \Biggl(0, 4D_t^\mathrm{opt}vl\sum_i^{m_n}S_i^\mathrm{para} - M^{\mathrm{cpu}}\Biggr) \\
    & T_\mathrm{update} = \frac{\sum_i^{m_n}S_i^\mathrm{para}}{F^\mathrm{cpu}}+\frac{D_t^\mathrm{grad}vl\sum_i^{m_n}S_i^\mathrm{para}}{B^\mathrm{h2d}}+\frac{D_t^\mathrm{para}vl\sum_i^{m_n}S_i^\mathrm{para}}{B^\mathrm{d2h}}
\end{align}

\textbf{激活值显存优化}：激活值显存节省通常采用两类优化：激活值重计算或者激活值卸载，相似地，两类优化对训练性能影响不同。

激活值重计算：激活值重计算包括两种，selective重计算和full重计算。selective重计算仅将attention部分激活值进行重计算，其他部分激活值保留，在反向传播时重新计算Q-K-V的生成矩阵以产生Attention的输入，重新计算attention以产生attention中间激活值，我们将该优化进行如下建模：
\begin{align}
    & M^{\mathrm{act}} = \left(vp+p-2r_{pp}-1 \right)\times\Biggl(\sum_i^{m_n}M_i^\mathrm{act}-M^\mathrm{Attention}\Biggr)\\
    & T^\mathrm{BWD} = T^\mathrm{BWD}+T^\mathrm{QKV}+T^\mathrm{Attention}
\end{align}
其中$M^\mathrm{Attention}$为Attention模块的中间激活值，$T^\mathrm{QKV}$和$T^\mathrm{Attention}$分别为Q-K-V生成矩阵计算耗时和Attention模块计算耗时。

Full重计算原理将一层transformer层进行重计算，只保留一层的输入，在反向传播时重新计算一层前向传播产生激活值，可以极大节省激活值显存占用。根据两类重计算设计特点对进行显存和性能建模：
\begin{align}
    & M^{\mathrm{act}} = \left(vp+p-2r_{pp}-1 \right)M^\mathrm{input}\\
    & T^\mathrm{BWD} = T^\mathrm{BWD} + T^\mathrm{FWD}
\end{align}
其中$M^\mathrm{input}$为一层输入占用显存大小。

激活值卸载：业界主流激活值卸载策略一般采用异步激活值卸载方式，其原理是前向传播时将每一层的激活值在下一层前向传播阶段进行异步卸载，反向传播时将每一层的激活值在前一层反向传播阶段进行预取，这种方式可以减少大量激活值显存占用同时引入更少计算耗时，根据该设计特定对异步激活值卸载进行显存和性能方面建模：
\begin{align}
\label{offload}
    & M^{\mathrm{act}} = \sum_i^{m_n}M_i^\mathrm{act}\\
    & T^\mathrm{FWD} = \max \Biggl( \alpha^\mathrm{offload} \frac{M^{\mathrm{act}}}{B^\mathrm{D2H}}, \beta^\mathrm{offload} T^\mathrm{FWD} \Biggr) \\
    & T^\mathrm{BWD} = \max \Biggl( \alpha^\mathrm{fetch} \frac{M^{\mathrm{act}}}{B^\mathrm{H2D}}, \beta^\mathrm{fetch} T^\mathrm{BWD} \Biggr)
\end{align}
其中$\alpha^\mathrm{offload}$和$\beta^\mathrm{offload}$分别为卸载时D2H和计算耗时增加系数，$\alpha^\mathrm{fetch}$和$\beta^\mathrm{fetch}$分别为激活值获取时H2D和计算耗时增加系数。

根据选择的显存优化策略代入其影响的基础性能模型中便可以得到相应显存优化对显存和性能的影响，从而有效评估训练效率。



\section{Experiment and Analysis}
\subsection{Experimental Setup}
Our experiments were conducted on two types of GPUs with detailed specifications listed in the table below. 
The distributed framework employed was Megatron-LM, and the software environment consisted of Python 3.8 and PyTorch 2.1.0.
\input{Table/5/GPUs}

\subsection{MoFa Performance Modeling Evaluation}
\input{Table/5/modeling-perf}
本节中，我们对MoFa的建模精度进行评估。评估过程主要选取以下3个典型模型：LLaMA2-70B，LLaMA3-405B和DeepSeek-V3-671B。LLaMA2-70B和LLaMA3-405B分别是100B量级以下和以上的主流dense模型，DeepSeek-V3-671B是目前主流的Moe模型。表x中展示了三个模型的关键架构参数。
我们利用MoFa对三个模型进行建模并和实际性能进行了对比。如Table.X所示, MoFa建模的输入包含集群硬件配置、采用的模型并行配置、采用的优化特性和故障容错配置。在Performance Evaluation一栏，我们展示了MoFa的建模结果。LLaMA2-70B建模了四个规模下性能，卡数分别为128，256，512，1024，可以看出在百卡规模集群例如卡数128时，建模精度为99.6$\%$，在千卡规模集群例如卡数1024时，建模精度为97.65$\%$。LLaMA3-405B和DeepSeek-v3-671B的建模精度分别达到98.73$\%$和97.72$\%$，说明MoFa建模精度较高。
此外，我们发现ETTR随着训练规模的扩大呈上升趋势，llama2 70B的训练规模从128卡增加至1024卡，ETTR由99.49$\%$提升至99.39$\%$。并且ETTR上升程度随着训练规模扩大逐渐变缓，从128卡增加至256卡时，ETTR增幅为$0.6\%$。从512卡增加至1024卡时，ETTR增幅为$0.07\%$.该现象的原因是在当前训练规模下，$t_{step}$增大和$t_{save}$降低所带来的正向收益要大于$W_{n}$增大导致故障率增加和$u_b$增大所带来的负向收益。但随着集群规模增大，负向收益所占的比重越来越大，导致ETTR增长程度变缓。


\input{Table/5/modelchoice}

\subsection{MoFa Tuning Evaluation}
真实的训练过程中，训练者一般会在固定大小的集群上进行训练。同时，为了保证训练loss一致性，训练者会选用固定的GBS。本节中，我们展示了固定集群规模和GBS大小的情况下，利用MoFa寻优最优的performance，以及对应的并行配置，优化特性和关键阶段信息。本节以LLaMA3-405B模型为例来说明MoFa寻优能力。我们选择了三种规模进行寻优，包括百卡级别规模（64卡），千卡级别规模（2048卡）和万卡级别规模的集群（8192卡）。同时，每个集群规模场景下，我们选择了小GBS和大GBS两类设置，分别按照0.25倍集群大小和1倍集群大小配置。
在MoFa Tuning中，我们展示了每个场景下前4组寻优配置，如tablexx所示。通过MoFa Tuning，训练者可以根据实际情况选择最优的配置，从而最大化的利用集群资源，加速整体训练过程。在百卡规模集群小GBS训练场景下，从性能提升角度考虑，建模得出Top1的配置相比Top2、Top3和Top4的性能提升分别是6.24$\%$，13.22$\%$和20.27$\%$。进一步，我们根据关键信息可以看出Top1相比Top2主要收益是来自Mbs的增大，增大Mbs虽然会增加PP耗时但算子耗时减少收益更多。Top1相比Top3主要收益是来自更小的计算耗时和TP耗时，相比Top4收益是更小的计算耗时和PP耗时。此外，在千卡规模或者万卡规模寻优下，由于引入DP，寻优会更加复杂。上述分析充分说明了训练系统具有高度耦合性，即硬件资源、模型结构、并行策略和优化特性等各个要素之间相互耦合，每个因素对不同的阶段产生不同影响，最终共同反映到整体性能上。MoFa Tuning System 以训练最小耗时为目标训练系统进行端到端性能寻优、系统性地识别各项要素之间的相关性以及各要素对最终系统性能的影响，体现出了MoFa的先进性和有效性。

\input{Table/5/search-perf}

\subsection{Analysis of Key Settings on Performance}
本章节中，我们以chunk数和优化器类型为例探究寻优过程中关键配置对性能的影响。
\subsubsection{Effect of $v$}
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.45]{figures/5/chunkeffect.pdf}
    \caption{Effect of chunk $v$.}
    \label{v-effect}
\end{figure}
一般来说，为了最小化1F1B中的PP Bubble，即由于PP等待导致的计算Bubble，训练者会将$v$设置到最大，即$v=L/p$。但根据\ref{ppwarmup}$\sim$\ref{ppcooldown}可以看出增大$v$会将PP通信次数和时延增大$v$倍。虽然Steady阶段可以采用PP Overlap，即\ref{PPOverlap}，来减轻PP通信时延，但Warmup和Cooldown阶段的PP耗时仍然会增加，因此有可能较大的$v$并不是最好的选择。为了探究$v$的影响，我们通过MoFa对不同的$v$下LLaMA3-405B训练性能进行了建模评估，如图\ref{v-effect}所示，卡类型选择为B，卡数固定为2048，4种GBS场景被选择用于分析。根据图\ref{v-effect}，可以看出不同GBS下训练时延均是随着$v$增大呈现先下降再上升趋势，这说明最优$v=8$而不是$16$，原因是由于$v=16$时暴露的PP耗时多于减少的PP Bubble。以$G_{bs}=2048$为例，$v=8$相比于$v=16$增加2.7s PP耗时，但只减少1s。此外，我们还可以发现随着$G_{bs}$增大，不同$v$之间的耗时相差越来越小，这是由于$G_{bs}$越大，PP Bubble越小，并且Warmup和Cooldown阶段占比变小导致增加的PP耗时占比也减小。

\subsubsection{Effect of Optimizer Optimization}
在静态显存中，优化器占比高达$80\%$，需要做优化器显存优化。不同的优化器显存优化对性能影响不同。本章节探究\ref{cpuadam}和\ref{distributed-optimizer}两种优化器显存优化对性能影响。以LLaMA3-405B训练为例，我们选择了两种场景：百卡规模下单DP和千卡规模多DP，以提供更全面的分析。表\ref{tab:optimizer-effect}展示了百卡规模下LLaMA3-405B 单DP Top3性能的并行策略，其中卡型选择为B，$G_{bs}=16$。可以看出在CPU优化器下，64卡即可部署LLaMA3-405B，否则至少256卡，这样会导致大量的PP Bubble，使得单DP性能衰减仅$50\%$。与此同时，我们也可以看出CPU优化器显存优化效果比分布式优化器更高，64卡部署所需显存相比256卡进一步节省了，因此，从单DP性能和资源考虑上看，CPU优化器是一个很好的选择。
在千卡规模下，我们分析了不同GBS下CPU优化器和分布式优化器之间的最优性能和显存，如图\ref{optimizer-compare}所示。可以看出，随着$G_{bs}=16$增大CPU优化器和分布式优化器的性能差距逐渐减小，从$9.6\%$降低至$0.4\%$，主要是因为$G_{bs}$越大优化器耗时占比越低。但从\ref{optimizer-compare}右图可以看出，CPU优化器显存上相比分布式优化器在显存上更有优势，在各个GBS下CPU优化器相比分布式优化器显存均可以额外节省大约$8.3\%$。因此，在像千卡、万卡这种大规模训练场景大GBS场景下，采用CPU优化器更有性价比。

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{figures/5/optimizercompare.pdf}
    \caption{Distributed Optimizer vs CPU Optimizer.}
    \label{optimizer-compare}
\end{figure}


\input{Table/5/optimizereffect}


\subsection{Cluster Configuration on Performance}
随着训练集群规模增大，集群扩展能力和节点形态对训练性能至关重要。本章节基于MoFa探索大规模集群线性度和节点形态对训练性能影响。
\subsubsection{Cluster Size}
本章节我们以LLaMA3-405B为例，通过MoFa Tuning，探究随着规模逐渐增大集群线性度变化，以及DP Overlap特性对线性度的影响。具体来说，我们通过MoFa寻优$G_{bs}=1024$和$G_{bs}=4096$两种场景下64卡至8192卡的最优性能，并按照如下公式计算了集群线性度，如图x所示。可以看出，增大$G_{bs}$并采用DP Overlap特性可以有效地提升集群的线性度。$G_{bs}=4096$带DP Overlap的线性度相比$G_{bs}=4096$不带DP Overlap、$G_{bs}=1024$带DP Overlap、$G_{bs}=1024$不带DP Overlap分别提升了$9\%$、$25\%$和$35\%$。

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.6]{figures/5/linearity.pdf}
    \caption{Analysis of Cluster Linearity.}
    \label{linearity-analysis}
\end{figure}

\subsubsection{Node Size}
目前超节点逐渐成为主流，超节点规模如何设计是一个重要话题。本小节以DeepSeek-V3为例，通过MoFa寻优说明超节点形态对Moe模型最优性能下EP设置和EP-Overlap特性的影响。
表\ref{tab:N-effect}展示了$G_n=1024,2048,4096,8192$下的不同超节点配置对最优EP的性能，其中固定EP Overlap优化开启，可以看出集群规模、超节点配置共同影响最优EP。具体来说，在$G_n=1024$和$2048$下，最优EP寻优为$e=128$，在$G_n=4096$和$8192$下，最优EP寻优为$e=256$。EP越大专家计算效率越高，算子时延越少，这从$Tcal$可以得出。此外，我们还能看出在节点卡数$N=32\sim256$的Tstep相差较小，差距$<4\%$，这说明超节点规模存在一定边际效应，效率提升比例越来越小。
此外，我们还在图\ref{ep-overlap}中探索了不同$N$下EP Overlap性能提升情况，可以看出随着$N$增大，EP Overlap收益更大，主要是因为$N$越大，专家计算耗时越低，一个Step中EP占比增加，通过EP Overlap可以减少比例变大的EP耗时，从而获得更大的收益。此外，我们还可以发现在$G_n=1024\sim8192$均可得到该结论，特别是在$N=64\sim256$时，可以获得$>17\%$的性能收益。

\input{Table/5/N-effect}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.6]{figures/5/epoverlap.pdf}
    \caption{Performance Improvement Ratio of EP Overlap}
    \label{ep-overlap}
\end{figure}


